Pretrained Language Models for Sequential Sentence Classification

As a step toward better document-level understanding, we explore classification of a sequence of sentences into their corresponding categories, a task that requires understanding sentences in context of the document. Recent successful models for this task have used hierarchical models to contextualize sentence representations, and Conditional Random Fields (CRFs) to incorporate dependencies between subsequent labels. In this work, we show that pretrained language models, BERT (Devlin et al., 2018) in particular, can be used for this task to capture contextual dependencies without the need for hierarchical encoding nor a CRF. Specifically, we construct a joint sentence representation that allows BERT Transformer layers to directly utilize contextual information from all words in all sentences. Our approach achieves state-of-the-art results on four datasets, including a new dataset of structured scientific abstracts.

==> related_old.tex <==
\accomment{need to shorten this now that we are submitting a short.}
\subsection*{Pretrained language modeling:}
Recent contextualized language models have shown promising results on many token and sentence level NLP tasks. \bert \cite{Devlin2018BERTPO} is among the most widely-adopted models and is based on a Transformer \cite{Vaswani2017AttentionIA} architecture that builds representations by jointly conditioning on both left and right context. Models finetuned using \bert representations produce SOTA results on a variety of NLP tasks including QA, NLI, and the GLUE benchmark. There are several challenges before we can apply \bert for document-level tasks like structured abstract sentence classification. Our proposed \ourmodel{} is novel in the sense that 1) it divides the context into smaller windows and applies BERT on each of them independently 2) instead of using a single {\tt{[CLS]}} token for prediction, it uses {\tt{[SEP]}} tokens separating two sentences to predict the rhetorical label of each sentence in the context.       

\subsection*{Extractive summarization:} 
Methods proposed for this task range from efficient but poorly performing word count based models \cite{Salton1996AutomaticTD} to relatively systematic but computationally expensive CNN/RNN encoders for entire documents \cite{Cheng2016NeuralSB}.
In this paper we present experimental results on the CSPubSumTest dataset  \cite{Collins2017ASA}. Due to computational challenges \dkcomment{Is this true?}, their model uses conventional global context features and encodes only target (label) sequences with an RNN. \ourmodel{} overcomes the computational challenge by applying recent self-attention techniques that can handle longer context more efficiently than seq2seq models that involve sequential computations. To the best of our knowledge, \ourmodel{} is the first attempt to efficiently encode an entire document into a neural sequence encoder to produce SOTA results on the CSPubSumTest dataset \dkcomment{Should check this pending actual results}.

\subsection*{Rhetorical structure:} 
Finally, we demonstrate \ourmodel's effectiveness on the task of recovering the rhetorical structure of abstracts. SOTA methods for this task, HSLN-CNN and HSLN-RNN \cite{Jin2018HierarchicalNN}, use CNN and RNN based sentence encodings followed by attention pooling and a CRF decoder to output globally optimal label sequences for the entire abstract. \ourmodel{} is novel in the sense that we improve the sentence encoder by adapting the \bert encoder for this sequential task, and we replace the CRF decoder with a more efficient multi-layer perceptron layer. This updated architecture 
results in state-of-the-art performance on both CS-abstruct and PubMed-RCT datasets.
